Wide Area Network Autoscaling for Cloud Applications

Modern cloud orchestrators like Kubernetes provide a versatile and robust way to host applications at scale. One of their key features is autoscaling, which automatically adjusts cloud resources (compute, memory, storage) in order to adapt to the demands of applications. However, the scope of cloud autoscaling is limited to the datacenter hosting the cloud and it doesn't apply uniformly to the allocation of network resources. In I/O-constrained or data-in-motion use cases this can lead to severe performance degradation for the application. For example, when the load on a cloud service increases and the Wide Area Network (WAN) connecting the datacenter to the Internet becomes saturated, the application flows experience an increase in delay and loss. In many cases this is dealt with overprovisioning network capacity, which introduces additional costs and inefficiencies. On the other hand, thanks to the concept of "Network as Code", the WAN exposes a set of APIs that can be used to dynamically allocate and de-allocate capacity on-demand. In this paper we propose extending the concept of cloud autoscaling into the network to address this limitation. This way, applications running in the cloud can communicate their networking requirements, like bandwidth or traffic profile, to a Software-Defined Networking (SDN) controller or Network as a Service (NaaS) platform. Moreover, we aim to define the concepts of vertical and horizontal autoscaling applied to networking. We present a prototype that automatically allocates bandwidth to the underlay network, according to the requirements of the applications hosted in Kubernetes. Finally, we discuss open research challenges.

==> Other/done.tex <==
%FIXME Berta: Please add the author list, people are more engaged when reviewing a paper and they see their names there. The most important position for young researchers (like you) is the first one, the most important one for senior researchers (like me) is the last one. This is a paper lead by Cisco, so Cisco deserves the last position. The author list should be you, Jordi, XXX, Albert C, XXX, Fabio. Please ask Alberto/Fabio how they would like to order the author list, you will go first, then I don´t care where I am placed (tell Fabio) and in my understanding Fabio should be the last one (this is up to them). In my opinion Jordi should go second, but if Cisco feels otherwise then change it.

%DONE Berta: Also, please check the template (or other papers) and add this:
%This work is supported by the Spanish MINECO under contract TEC2017-90034-C2-1-R (ALLIANCE) and the Catalan Institution for Research and Advanced Studies (ICREA).

%FIXME: Jordi Please rewrite based on the new focus, intro and experiments.


%FIXME Jordi -> Please complete

%FIXME Jordi: Please add a paragraph here. Explain that orchestration is needed to to support fine-grained compute granularity, explain the main orchestration mechanisms (k8s and others). Also, describe the service mesh and istio/emboy, this is programmable data-center networks. Explain that this programmability only applies to the compute domain.


%FIXME Jordi: please rewrite the paragraph below in line with this new introduction. Say that this is not new, but describe the differences with existing approaches. Maybe the difference is that the requiremetns do not come staright from the application? Also discuss B4.



%FIXME Jordi->Explain the first use-case and then the second one.


%FIXME Jordi/Berta: This section needs to be entirely rewritten, please use the following structure:

%FIXME Jordi/Berta: First add a new plot showing the end-to-end architecture, this means the cloud controller, the SDN controller and the end-user network (and the user, a mobile phone or whatever). Then draw the proper 'arrows' showing how the cloud orchestrator controls the cloud, the SDN the network, etc. And then explain it step by step.

%FIXME Jordi/Berta: Then say that we focus on network horizontal and vertical scalability. Then add two 'sections' \textbf{Network Horizontal Scalability:} \textbf{Network Vertical Scalability:}and properly define them. Try to come up with a definition that applies now and in the future. Also, describe how they are different from cloud scalability.


%FIXME: Jordi, this is quite messy. Please rewrite, try to provide a story. 


%FXIME: Jordi please rewrite, it is quite messy. Try to elevate the text. Use the format "title: XXXX". 

%FIXME: The first item is well-understood, please say that other approaches are possible, prediction, etc. Say clearly that there is plenty of literature on this topic. 

%FIXME Jordi: The second item is relevant, discuss that fine-grained (perfect) granurality to achieve 100% utilisation requires traffic modelling and shaping, otherwise bursts of traffic will produce congestion. This is a well understood field. Also, allowing for very fine-grained granurality at the overlay controller requires optimization techniques to make good use of the underlay resources.

%FIXME Jordi: The horizontal autoscaling one, please think about it, let´s discuss it a bit more.

%FIXME Jordi: The last one is great, but please rewrite, it is messy.

%FIXME Berta - Fig 3, provision or capacity update? Provision means establish. Caption, "Overlay controller responste time". 

%FIXME: Berta please complete REFs, etc. Also, never use the passive form when writing in english. And always use short sentences. In Spanish we are used to very long sentences, connected with 'y' 'pero' or commas. Don´t do that in English, just sentence. sentence. sentence, telegraphic. 


%FIXME Berta - Fig 2, the blue line does not start at 0 and/or end at 1, why? Same for the red, orange lines, please check the Y axis ranges. Also, use stronger lines (more width) and try to plot them in black and white. Also the caption "Kubernetes Controller response time"

%FIXME2: Discuss in call.
%FIXME2: Yes, keep it, discuss in call. 
%FIXME2 BEFORE SENDING >> note that this is reducing the configuration time , of something that is usually provisioning/configuration (when you change the rate limiting of a customer in packet fabric)
%FIXME2: Yes, keep it, discuss in call. EXPAND: if the underlay can give info to the underlay like BW, reduntatn path, you can do more stuff (do not mix with does HZTAL make sense)

%FIXME2: Expand, please explain why it is crucial? Also explain what we do in this paper and what we think makes more sense to do in the future.
%FIXME3: FIXME2 still holds.

%FIXME2: This needs to be explained WAY better, please explain why in a point-to-multipoint this does not work. i.e. a cloud connected to different WANs or networks

%FIXME3: Please cite openstack, kubernetes, envoy...

%TODO: add a new section about multiple applications: say that if we have multiple applications, and one of them scales up a virtual cirtuit, this can impact the others. In other words, the overlay has to take into account the impact of scaling the bandwidth with respect to the total available bandwdith. 
%Berta: review section

%TODO: put it in a positive way, there is the option to make it more granular

% TODO: add a discussion that reaction time now is faster. It is not common to hear that provisioning time needs to decrease. Are current protocols fast enough for the new requirements (i.e. match autoscaling time of kubernetes)? Conider that we do not want to autoscale only for a spike.

%TODO: add that CNWAN provides a link between the application and the network. CNWAN: (i) helps identify which cloud applications have networking needs (eg. differenciate between a compute intensive application and a video server), (ii) propagates cloud autoscaling events to the network, and (iii) quantifies the amount of extra bandwidth required (scaling factor)
%Berta: review

% TODO: Fig. 3 add a moving average of the traffic, specify when the app starts scaling up
% TODO: Detail exactly that the bandwidth gets reserved shortly \emph{before} the traffic increases, highlight that this is proactive. 
% TODO: Mention that in case that the traffic didn't increase that much, we can quickly scale down afterwards.
%Berta: review, is this needed?

%TODO: say clearly that usually the scaling is reactive, the most notable example are techniques in elastic optical networks. Say here we want to be proactive. This makes it possible to adapt to changing demands. 

%Done Berta: digues directament els diferents steps que hi ha disponbiles, i que estan en el rang que surt a la grpafica, eg. in the following steps: 10, 20, 50 Mbps 
%Done Berta: first say how you started the experiment: we start with a link of XX Mbps start injecting traffic to...
%Done Berta then explain what happens: traffic starts increasing and k8s starts creating reaplicas. Then when the number of replicas is XXX this triggers an autosacling event (corregeix segons el que ho faci disparar). És més o menys el de sota però una mica més de detall. We can see that shortlly after the number of replicas crosses the XX threshold, the capacity is increased from X mbps to Y mbps (around XX s)
%Done? Berta: fes més èmfasi en el before, sé que sóc pesat, és perquè quedi més clar. Digues que we can see that the network provisions capaticy before when traffic is greather than 100 Mbps, aprox


%FIXME3: Please make it clear that optical auto-scaling does not interface with the cloud, but rather they are either customer subscriptions or based on traffic monitoring mechanisms. 

%BERTA: Review Dave's comments
% Fabio's feedback:
%JORDI: rewrite to it does not seem that the scale down is in the graph


%FIXME3: This needs to be expanded further (below) and explain it better. Put a more specific example using WAN and discuss also the financial reasons behind this. If need please let me know and we can have a quick chat.

%FIXME3: Please write the absolute time, so 0:30, then 1:30, then 2:30. 

%FIXME3: This paragraph below is a mess and does not make any sense, please heavly, if needed please let me know and we´ll have a quick chat.

%FIXME3 Below: I don´t understand anything, what are you trying to say? Explain WAY better please :)

==> Other/old_text.tex <==
%ABSTRACT


%alternative: say the problem is resource efficiency	
%and measure key performance metrics such as the delay to increase the bandwidth of a link.



%	Kubernetes provides a versatile and robust ways to host applications at scale. By being an open source platform for managing lightweight VMs, referred to as containers, it provides a framework to run distributed systems with a large and growing ecosystem supporting it.
	
%	Although this technology is usually deployed in conjunction with software-defined Wide Area Networks (SD-WAN), they are usually unaware of each other, missing out optimisation opportunities.
	
%	As a part of the Cloud Native SD-WAN (CN-WAN) open source project, this paper aims to define the concepts of vertical and horizontal autoscaling applied to networking. In addition, it provides a demonstration of vertical network autoscaling by automatically allocating bandwidth on a virtual circuit on the SD-WAN underlay in order to meet the requirements of the applications hosted in Kubernetes.
%    It shows its viability while discussing the outcome, stating emerging remarks and discussing future lines of work.

%OTHER
%In the cloud domain, autoscaling is a feature to dynamically adapt the amount of compute resources to the current load, as a way to improve efficiency and optimize cost. Usually, cloud autoscaling works in two axes. The first, vertical autoscaling (also known as scale up or down) refers to adding more resources to an existing cloud instance, such as CPU, memory or I/O resources. The second, horizontal autoscaling (scale out or in) involves adding new cloud instances to divide a workload among them. 


%FIXME2 (below): This is great related work, please -partially- this content to section 2. 

%Regarding vertical autoscaling, we leverage modern API-driven ISP providers  \cite{PacketFabric} to dynamically allocate the bandwidth of WAN tunnels depending on the autoscaling status of cloud applications, i.e. if the application scales out, we trigger an API call to increase virtual circuit bandwidth. We must remark that there is a significant research around allocating bandwidth demands in networks, like the Routing and Spectrum Allocation problem in optical networks \cite{elasticOpticalNetsTutorial}, the Virtual Network Embedding problem for guaranteed bandwidth \cite{VNE_review}, or algorithms to scale Virtual Network Functions for a given load \cite{engine}. In our case we take a proactive approach and directly transfer application demands to the network. \textbf{expand differences / not sure these works are directly related}. 

%FIXME2 (below): This is great related work, please -partially- this content to section 2. 

%With respect to horizontal autoscaling, we make use of the programmability of both cloud platforms and modern SD-WANs to transfer the networking requirements of cloud applications (e.g. latency, bandwidth) to the SD-WAN controller, so the latter can select the best path. There is extensive research on communicating application requirements or QoS needs to the network. The most closely related works focus on extending the socket API in order to support QoS requirements. However, in our case we don't modify the socket API but read the application requirements from cloud orchestrator and how to identify application to the SD-WAN controller. Other similar research focuses on the user-to-network segment \cite{pavingFirstMileQoS}, while we focus on the WAN part, or communicating cloud orchestrators across the WAN \cite{RodriguezYaguache2019EdgeComputingContainer}, or only deal video streams \cite{qosVideoStreaming}.
%we can say we offer a middle ground with the abstraction: only what you need, but not in deatil...? otherwise complex to do in the data plane


%INTRO:
%BERTA: revisar
%In the cloud domain, autoscaling is a feature to dynamically adapt the amount of compute resources to the current load, as a way to improve efficiency and optimize cost. Usually, cloud autoscaling works in two axes. The first, vertical autoscaling (also known as scale up or down) refers to adding more resources to an existing cloud instance, such as CPU, memory or I/O resources. The second, horizontal autoscaling (scale out or in) involves adding new cloud instances to divide a workload among them.

Therefore, we propose  propagating cloud autoscaling events to the network that connects the datacenter with the end-users. This way, the network can scale according to the requirements of the cloud. More specifically, we consume scaling events from a cloud orchestrator and relay them to an SDN controller in odrder to: (i) increase virtual circuit bandwidth using an underlay provider, and (ii) identify application flows to appropriately steer them  in the network. 

The rest of this paper is organized as follows: first we define vertical and horizontal network autoscaling and present a general architecture to support such new features. Then, we experimentally prototype and analyze two real-world use-cases of both network autoscaling scenarios. Finally, we take advantage of both experiments to derive open research challenges in this field. 


%extending benefits of cloud to networks


%\textbf{REMOVE?}This new relation between NetOps and DevOps would not only provide an optimal application utilisation but also it would reduce the development complexity while bringing the opportunity to automate their delivery. \textbf{REMOVE?}


%Still, there is no real cooperation between these two services to match the network characteristics to meet the application and services needs to achieve a strong resource optimization. This link creation between NetOps and DevOps would not only provide an optimal application utilisation but also it would reduce the development complexity while bringing the opportunity to automate their delivery. 



%Previous efforts to make networks more elastic have been made. G. A. Carella et al.\ \cite{engine} leverage Network Function Virtualization to reduce the complexity of managing Network Services.  D.Niu et al.\ \cite{videodemand} define a predictive algorithm to reserve bandwidth for a video-on-demand application. In cloud environments in particular, T.Lorido et al.\ \cite{review_techniques} make an extensive review on autoscaling techniques applied to applications in cloud deployments. All these have two aspects in common: the need to adapt the existing resources in order to provide optimal application experience and the fact that to make the network scalable this needs to be software defined. 

% However, all these solutions have a reactive or predictive approach when trying to adapt the network to the desired state. It is crucial to move towards matching Kubernetes’ elasticity in a more proactive solution in order to reduce delays caused by changes in demands. And to do so it is necessary to enable cooperation between the application and the network.




%We present a prototype with \textbf{FIXME Albert: complete with details of the prototype} to understand the performance as well as main bottlenecks. With this feedback, we discuss the main research challenges in this new field.

%For this reason in this article two key concepts are defined: horizontal and vertical network autoscaling. 
%As a part of the Cloud Native SD-WAN (CN-WAN) open-source project \cite{CN-WAN}, an implementation of vertical network autoscaling is demonstrated. 
%This solution focuses on extending SD-WAN features to make it more aware of the scaling information provided by Kubernetes naturally. In particular it demonstrates how an SD-WAN can autoscale in terms of the desired replicas in a Kubernetes cluster hosted in a cloud environment. 

%Leveraging the existing CN-WAN extensions, an adaption has been made to communicate the SD-WAN controller with an underlay provider to adjust the bandwidth requested by an application in an automated way. This communication is based on the programmability of API-driven underlay providers.

%As a result, this paper shows the outcome of this implementation, providing insights on the channel bandwidth fluctuation in terms of resources requested by the cloud application. In addition, a study of the network adaptation latency is stated along with the discussion about the requirements that have risen in network autoscaling.

%FIXME2 Berta: Rewrite paragraph below once the main contents of the paper is finished.
%The remaining of this paper is structured as follows: to begin with the autoscaling network paradigm is defined as well as the scenario used. It is followed by exposing the results of implementing vertical network autoscaling. In the fourth section, related work is disseminated to provide a broader context. Finally, in the last two sections important remarks are discussed as well as the conclusions.


%With this, autoscaling events detected by the cloud orchestrator only propagate within the compute domain (i.,e, datacenter), but not to the networking domain that connects the application with the end-users. This fundamentally limits the autoscaling properties of the cloud, since an application can scale up to support higher loads, but the connection towards the uses remains unchanged, which might cause congestion. Similarly, inefficient use the network resources occurs when the application scales down. 


%This will enable matching the requirements of applications and services with the resources offered by the network, increasing the resource efficiency. 

%In this paper we explore how to propagate cloud autoscaling events to the network that connects the datacenter with the end-users. 


%. Then, we experimentally prototype and analyze two real-world use-cases of both network autoscaling scenarios. Finally, we take advantage of both experiments to derive open research challenges in this field.

SEC II: AUTOSCALING ARCHITECTURE

%The following paragraphs attempt to define the concepts of vertical and horizontal network autoscaling.

%This paper sets a new perspective on autoscaling networks. By defining the concepts of vertical and horizontal autoscaling in SDNs it brings a new focus on optimizing network resources by providing the best cloud application performance.

%It is centred in providing a coordination between the DevOps, in charge of configuring and operating the Kubernetes infrastructure, and NetOps, responsible of maintaining the SD-WAN connectivity. It also demonstrates vertical autoscaling in a simple scenario where the cloud elasticity is matched with the optimal network resource optimization.

%In order to carry out a vertical network autoscaling demonstration, the Cloud Native SD-WAN (CN-WAN) open source project has been leveraged.
%The CN-WAN open source project creates an approach on how SD-WAN controllers can use Kubernetes metadata in order to adjust the network to fit better the requirements (such as routing traffic through appropriate channels or adjusting the channels to match the traffic).

%To enable this cooperation, the project is divided into three main components, as shown in figure \ref{fig:Overview}. 

%TODO: decide if related work is relevant here
%Previous research has focused on propagating application information across specific segments, like the user-to-network segment \cite{pavingFirstMileQoS}, or across cloud orchestrators in a WAN \cite{RodriguezYaguache2019EdgeComputingContainer}, or proposed solutions for specific applications, like video streams \cite{qosVideoStreaming}. On the other hand, our approach is application agnostic and we don't focus on a specific network segment.  


%The autoscaling concept rose along with cloud computing and Kubernetes.
%Containers have become the de-facto standard for delivering applications packaged and portable to any operating system. These lightweight, standalone, executable packages of software make the applications run quickly and reliably. 
%They contain all the requirements needed to run an application and are properly isolated between each other, though communication can be established using the proper channels.

%Kubernetes is an open-source platform that manages container workloads. Its services allow an easier declarative configuration and automation while providing scaling, failover, load balancing tools and deployment patterns to the applications.

%Kubernetes performs this management through pods, the smallest deployable objects. One pod can contain one or multiple containers managed as a single entity that share resources.

%Focusing particularly on scaling, Kubernetes allows the adoption of vertical and horizontal autoscaling. 
%Vertical pod autoscaling allows the containers to dynamically adjust in CPU and/or memory requests and limits, providing efficiency inside cluster nodes, fewer maintenance expenses and the elimination of tasks to determine the appropriate value for those features.
%However, horizontal pod autoscaling \cite{HPA} scales the number of pods in a controller depending on specific metrics set. These metrics can be per-pod, such as CPU and memory, or customized. 
%Multidimensional autoscaling is also viable and incorporates both, vertical and horizontal autoscaling.

%Due to programmable networks, the Kubernetes autoscaling paradigm can be translated into network autoscaling terms. In this case, horizontal autoscaling is defined as replicating a channel into other disjoint channels that have the same resources. In parallel, vertical autoscaling is defined as dynamically adjusting the resources of a channel in order to meet the desired requirements. 

%This way, we avoid overproivsioning a  virtual circuit to fulfill a particular SLA, 

%In vertical network autoscaling, we can only increase the bandwidth of a virtual circuit. In this situation, it can happen that we oversubscribe this virtual circuit to fulfill a particular SLA. 


%In other words, if we can change our underlay provider, we can optimize resource usage.

%Furthermore, it may happen that a tunnel in the network becomes congested to due increased load of this application. In this case, the SDN controller can keep this QoS requirement (autoscale) by redirecting part of the load to another path that is less congested. 
%FIXME3: I have removed the sentence starting with "Furthermore," because is this truly autoscaling? or simple overlay management?


SEC III results
%A little later, we can sSince We defined a network load of 1 Mbps per Kubernetes replica,
%Once the number of replicas is greater than 50 a WAN autoscaling event is generated. 

%Previous text
%An important remark is that this capacity update is proactively triggered, meaning that the virtual circuit upgrade is processed before the network traffic is greater than 100 Mbps. Note that the proprietary overlay SDN controller used in this experiment can scale the bandwidth in the following steps: 50, 100, 200 Mbps.

%FIXME3: I don´t understand the latest sentence, pelase clarify




%In particular, when the target replicas in Kubernetes become grater than 50, it triggers a capacity update of the virtual circuit which starts \emph{before} the traffic load reaches the network. We can see that the network allocates more bandwidth on the virtual circuit before the traffic is greater than 100 Mbps.

%FIXME3: What is the purpose of this sentence (below?), it is not related to any experiment. If the sentence has a purpose please don´t remove it and better align it with the text.
%Finally, in case that the traffic increase does not take place, the network can scale down in sync with the cloud, in order to avoid overprovisioning the connection. 

%The plot shows how the bandwidth allocated to the virtual circuit approximately matches the load produced by the increasing throughput. 
%The generated traffic triggers more replicas deployed which in turn trigger autoscaling events to increase the connection capacity. 
%Please note that the overlay SDN controller offers a granularity of 50 Mbps, meaning that bandwidth can be scaled-up or down in steps of 50 Mbps.
%A relevant observation is that the coarse granularity offered by the overlay network controller only allows to scale-up the bandwidth in fixed steps such as 50-100 Mbps or 100-200 Mbps. This produces an inefficient use of the resources. 


%propagate autoscaling events from the cloud to the network that interconnects the cloud with the end-users. 

%The first one, the Operator, is a Kubernetes operator that monitors externally exposed services in the cluster looking for SD-WAN related metadata. An example of metadata would be the annotation of ‘replicas’ to indicate what type of traffic can the SD-WAN expect. Then, the operator extracts the externally exposed IP address, port and metadata and it publishes it in a service registry.

%The second component is the Reader. Its mission is to periodically poll the service registry in order to keep track of any update related to the exposed services and metadata. Upon a change in the registry, it sends an event towards the Adaptor, the last component.

%To end the cycle, the Adaptor is in charge of translating this registry update to actually providing changes to the network to adapt to it. In the example mentioned before, it would update SD-WAN controller policies for the services specified (e.g., Video should go through this particular link).

%Our proposal is to extend the CN-WAN project to not only be able to modify SD-WAN policies in the controller but also to modify the underlay circuits. To do so, another Adaptor is created that serves as a bridge between the reader and the underlay of the SD-WAN. For the vertical network autoscaling purpose, the Adaptor implemented matches Kubernetes elasticity by modifying the virtual circuits. 
%In other words, when more replicas or resources are invested in Kubernetes the network adapts by allocating more bandwidth on the used circuits.


%As a SDN, an SD-WAN proprietary solution has been implemented and all the CN-WAN components have been integrated with the solution, including the modified version of the Adaptor. \textcolor{red}{As a cloud provider and service registry, a proprietary solution also has been chosen. Explain better??}

%The underlay is based also on a proprietary solution that delivers connections through their network-as-a-service platform. These connections can be configured to collocations, private clouds or other environments in terms of minutes while also allowing scalable bandwidth. This solution has been chosen due to the simplicity in API programmability which can be effectively connected to the Adaptor. An important mention about the underlay is the bandwidth allocation granularity. The virtual circuit’s bandwidth is a discrete function, meaning that sometimes there will be cases of small overprovisioning. In our scenario the underlay consists in a virtual circuit with up to 100Gbps of bandwidth. 

SEC V: RELATED WORK

%In this section we review some of the most relevant literature for this article.

%\subsection{Cloud Autoscaling}
% autoscaling is compute!!!


%On the contrary, we take a proactive approach because we directly leverage data from the cloud orchestrator instead of trying to predict the application bandwidth.

%FIXME3: Paragraph above, it is wrong (I think).I understand that the papers cited in the related work are for the cloud, not for the WAN. If this is the case then say it. If this is not the case then also say it, it is confusing either way :)

%In addition, in cloud scenarios the Kubernetes autoscaling features also need to be contemplated. 
%Authors of \cite{cloud_elasticity} provide an exhaustive review and classification of existing cloud computing elasticity techniques and purposes and state research challenges derived from that. Our work intends to set the baseline for autoscaling networks with the intent of optimizing the network resources necessary to match  the flexibility that is provided in the cloud environments. 


%\subsection{Dynamic Bandwidth Allocation}

%FIXME3: say the network is allocated INSIDE the DC

%Allocating bandwidth demands to a specific network connection is a well known NP hard problem, usually know as virtual network embedding \cite{VNE_review}. There is also a similar problem in optical networks, the Routing and Spectrum Allocation problem \cite{elasticOpticalNetsTutorial}. However, most research focuses on allocating bandwidth in specific scenarios, like datacenter networks \cite{predictable_datacenter_networks}, inter-datacenter connections \cite{costMinimizingBWGuarantee}, for virtual network functions  \cite{VNF_ML}, or video streaming \cite{videodemand}. 
%FIXME3: saay we focus on WAN and not a specifi application
%In our case, we are do not focus on a specific networking scenario,
%YES >>>> and we make use of existing knowledge from the cloud to integrate it in the network policies. 
%This avoids making load predictions or setting thresholds and its associated uncertainty.

% ORIGINAL TEXT
%Allocating bandwidth in specific network links is a well known NP hard problem in the area of virtual network embedding (VNE). Typically virtual networks have set requirements that need to be satisfied by a mapping process. In \cite{VNE_review} a survey and classification VNE algorithms. Previous literature of bandwidth allocation includes \cite{predictable_datacenter_networks} which is based on the hypervisor provided by virtualization to shape the traffic. 
%D.Niu et al.\ \cite{videodemand} define a predictive algorithm combined with multiplexing techniques in order to reserve bandwidth for a video-on-demand application. On a similar note, \cite{VNF_ML} uses machine learning  to predict VNF workloads for reserving bandwidth for posterior uses. While these solutions improve QoS, none of these leverage existing knowledge from Kubernetes to integrate it in the network policies. Our work is focused on autoscaling networks based on certain events provided by the Kubernetes controller without having to make load predictions or setting thresholds, which would add uncertainty or losses.
% ORIGINAL TEXT


%\subsection{Translating Application Requirements to the Network}

%FIXME3: Below, I think the paragraph is great, but please clarify the first sentence. Explain better what is the relation between extending the socket API wrt. what we are doing.
%Finally, for the case of communicating application requirements to the network, i.e., QoS, the largest body of research focuses on extensions of the socket API, either with new options or flags \cite{socketIntents}, protocol-independent APIs \cite{neatProtocolIndependentInternet}, or eBPF \cite{beyondSocketOptions}. Contrarily, we do not modify the host stack but use API-driven interfaces to identify flows and map them to the required QoS demands. Other works in similar direction to ours focus on the connections between end users and ISPs \cite{pavingFirstMileQoS}, radio networks \cite{policyBasedQoSStreamingServices}, or inter-datacenter connections \cite{RodriguezYaguache2019EdgeComputingContainer}, while  our proposal is centered on cloud applications and the network immediately after the datacenter. A more recent  proposal suggests merging the L3 stack with the L7 stack (i.e. service meshes), in order to increase performance and application awareness in the network \cite{fullStackSDN}.


SEC VI: RESEARCH CHALLENGES  


% PROVISIONING TIME
%On the same note, another improvement field would be the reduction of the time needed for modification of the bandwidth of the virtual circuit. 
%time between Kubernetes detecting and provisioning the replica, and consequently avoiding saturating the channel for a few seconds.
%SDN control protocols should be on par with kubernes delays


% NETWORK TOPOLOGY
%The last important remark is the topology of the system. The solution discussed in the paper is optimal in scenarios where there is a bottlenecked channel such as in cluster-to-cluster deployments. However, it raises the question about how the channels should be treated in other network topologies such as point-to-multipoint scenarios. Additional information about traffic location might be needed in order to scale the appropriate one. To do so, existing traffic monitoring techniques could be employed but at the cost of dealing with encrypted traffic. Another different perspective could be tracking the incoming connections in Kubernetes, adopting a more proactive position. Or in a more conservative scenario all the channels could increase their capacity until the actual location of the increased demand is located and then readjust all the overprovisioned links.


%UNDERLAY PROPERTIES
%Thus, some horizontal network autoscaling options are tightly linked with the ability to control the underlay hardware. 
%When it comes to the underlay, is where the term horizontal network autoscaling fits. Requesting a bandwidth modification from Kubernetes to the overlay does not assure redundancy since it is unaware of the traffic management that the underlay is providing. For this reason, defining horizontal autoscaling as duplicating channels with the same resource characteristics must be tightly linked with being able to control the underlay hardware. 

%\section{Discussion and Concluding Remarks: Open Research Challenges}

%In this section we describe several future research challenges.

%The softwarization of the WAN and the advent of connectivity service providers that are exposing APIs to dynamically provision underlay capacity, together with the development of an application-to-network API makes proactive autoscaling of WAN resources as easy as autoscaling compute and  memory. This is a very significant improvement, compared with the status quo of overprovisioning WAN capacity to address peaks of demand, as well as from solutions that monitor network utilization reacting to congestion and saturation. We conclude this paper with a list of future research challenges that are worth further investigation.   



%\textbf{Bandwidth Estimation:}  regarding vertical network autoscaling, it is crucial to do a proper estimation of the bandwidth required by each \emph{compute} replica, in order to maximize efficiency, prevent congestion or avoid overprovisioning bandwidth, and its associated cost. While in our prototype we let the user select this parameter, it would be much more accurate to automatically estimate this parameter, to adapt to applications that have different bandwidth demands during their execution time. There is extensive research on bandwidth estimation \cite{bwEstSurvey}, with monitoring tools or prediction algorithms, either linear \cite{linear_prediction}, or non-linear prediction \cite{nonlinear_prediction} models. Additional research is needed to understand how such existing techniques can benefit from having information from the cloud orchestrator.

%After the implementation of a vertical autoscaling network some important remarks have to be mentioned. First of all, it is crucial to do a proper estimation of required bandwidth of a Kubernetes replica.This value, configurable in the Adaptor, could be set following two approaches, either it could be freely configured by the developer or it could be estimated using monitoring or prediction algorithms. Many solutions are proposed in literature for predicting traffic, mainly divided in linear prediction \cite{linear_prediction} and non-linear prediction \cite{nonlinear_prediction} models.



%FIXME3: This paragraph below is a mess and does not make any sense, please heavly, if needed please let me know and we´ll have a quick chat.

%\textbf{Underlay Granularity:} the granularity of the underlay, that is, the different underlay bandwidth options that the SDN controller can request (10, 50, 100 Mbps, etc) is key to avoid overprovisioning and use resources more efficiently. 

%MORE CLEAR
%In the future, as bandwidth becomes more granular, knowing the application bandwidth in advance will  not  be sufficient to achieve high tunnel utilization, because sudden traffic bursts may create congestion. Hence, we will require traffic modeling and shaping techniques \cite{trafficModelling} to adapt to fast-changing traffic dynamics.



%\textbf{Provisioning  Time:} in the context of underlay providers, the maximum bandwidth of a tunnel, or rate limiting, is a setting that belongs to the control plane. As such, it is typically configured few times, and its provisioning time, i.e., the time until the setting takes effect, is not considered relevant. However, it is  interesting to note that in recent years this time has become significantly faster, changing from months to tenths of seconds \cite{PacketFabric}, making this setting much more dynamic. 

%Ideally, in our scenario this provisioning delay (currently around tenths of seconds) would need to commensurate with the reaction time of the cloud autoscaling engine (currently seconds), in order to avoid under-utilization or service disruption. In parallel, this raises the question if current control plane protocols are fast enough to support such dynamics.




%TODO: say that changing the path is relevant from a business model perspective. If you can only do vertical autoscaling, it can happen that you oversubcribe the network to fulfill a particular SLA. On the other hand, if you can dynamically choose from different providers you can adapt better to sudden increases in load. Hence, you are using resources more efficiently, and this translates to a cost reduction.


%FIXME3: Below, I think (nwo) below that this does not make sense. With Segment Routing, LISP, openflow, you have all the detaisl, right? If there is an underlay parameter for which we are certain that the overlay has no control then say it and leave the paragraph, otherwise let´s remove the paragraph.
%JORDI: fora perquè només és una característica i en tenim de més importants
%\textbf{Underlay Path Properties:} since the SDN controller may not be aware of all the characteristics of the underlay tunnels, this may affect the ability of network autoscaling to fulfill certain requests. For example, consider a scenario in which an application asks for redundant paths, as a different way to autoscale the network. This may not be possible depending on the SDN network underlay configuration. Thus, if the underlay can expose additional information to the SDN controller, like redundant paths or latency measurements, network autoscaling can offer more advanced features.





%FIXME3 Below: I don´t understand anything, what are you trying to say? Explain WAY better please :)

%\textbf{Application Diversity:} in environments where multiple applications share the same connection, autoscaling a single one can impact the performance of the others. Thus, the overlay should account for this diversity when autoscaling, considering the total available bandwidth and the autoscaling requirements of the other applications.



%\textbf{Network Topology: } our solution is designed for scenarios with point-to-point connections, because we can directly scale up the affected connection. In other words, when there is only one tunnel towards the datacenter, it is trivial to select which virtual circuit needs an increase in bandwidth. 

%However, consider a topology with the datacenter serves multiple access networks, each served by different overlay circuits. In this case, upon a surge in application traffic, and from the perspective of the cloud orchestrator, we don't know which virtual circuit needs additional bandwidth. Hence, we need more information about the traffic to determine which connections should be scaled. For example, we could employ traffic monitoring techniques, or take a more proactive approach by tracking the incoming connections to the cloud datacenter. Finally, a more conservative solution would be increasing the capacity of all the virtual circuits until we can determine the connection with increased demand, and then readjust the rest. 


%\textbf{Billing Model:} WAN autoscaling affords a new consumption model for WAN capacity where bandwidth is provisioned (and de-provisioned) on demand in quasi real time, rather than through overprovisioning. The billing model offered by today’s underlay connectivity providers reflects that consumption model offering increasing SLAs (such as 1, 10, 50 Gbps) typically billed on a monthly base. WAN autoscaling may drive the introduction of a new billing model where WAN consumption is billed on demand. We believe this may lead to a more efficient use of network infrastructure resources for the service provider that will in turn be reflected to a lower cost for the end user. Future work in this area should include a detailed analysis of billing models for WAN autoscaling, and their comparison with current billing models. 


%After the implementation of a vertical autoscaling network some important remarks have to be mentioned. First of all, it is crucial to do a proper estimation of required bandwidth of a Kubernetes replica.This value, configurable in the Adaptor, could be set following two approaches, either it could be freely configured by the developer or it could be estimated using monitoring or prediction algorithms. Many solutions are proposed in literature for predicting traffic, mainly divided in linear prediction \cite{linear_prediction} and non-linear prediction \cite{nonlinear_prediction} models.

%MORE CLEAR
%In the future, as bandwidth becomes more granular, knowing the application bandwidth in advance will  not  be sufficient to achieve high tunnel utilization, because sudden traffic bursts may create congestion. Hence, we will require traffic modeling and shaping techniques \cite{trafficModelling} to adapt to fast-changing traffic dynamics.

%TODO: say that changing the path is relevant from a business model perspective. If you can only do vertical autoscaling, it can happen that you oversubcribe the network to fulfill a particular SLA. On the other hand, if you can dynamically choose from different providers you can adapt better to sudden increases in load. Hence, you are using resources more efficiently, and this translates to a cost reduction.


%FIXME3: Below, I think (nwo) below that this does not make sense. With Segment Routing, LISP, openflow, you have all the detaisl, right? If there is an underlay parameter for which we are certain that the overlay has no control then say it and leave the paragraph, otherwise let´s remove the paragraph.
%JORDI: fora perquè només és una característica i en tenim de més importants
%\textbf{Underlay Path Properties:} since the SDN controller may not be aware of all the characteristics of the underlay tunnels, this may affect the ability of network autoscaling to fulfill certain requests. For example, consider a scenario in which an application asks for redundant paths, as a different way to autoscale the network. This may not be possible depending on the SDN network underlay configuration. Thus, if the underlay can expose additional information to the SDN controller, like redundant paths or latency measurements, network autoscaling can offer more advanced features.

==> Other/original_intro.tex <==
\section{Introduction}\

%In the last decade, software-defined networking (SDN) in a wide area network (WAN) has widely increased network automation. SD-WAN has allowed the separation of the data and control plane, allowing higher, dynamic and cost-effective performances. Its ability to support multiple underlay connection types, being able to perform dynamic path selection and integrating other third-party services with a single pane of glass controller are some of the main benefits that have increased its popularity.

During the last decade, Software-Defined Networking (SDN) has enabled programmability to network operation and management. By exposing expressive northbound APIs, the underlying physical network infrastructure can be controlled dynamically, offering unprecedented dynamic and quasi real-time network control. Recently, several commercial networking scenarios have embraced the SDN paradigm, this has resulted in a new breed of networking solutions. Notable examples of this are SD-Wide Area Network \cite{B4paper, wanSdnDataTransfers}, SD-Access Networks \cite{sdaPaper, ethaneSDNenterprise} and SD-Wireless \cite{sdWirelessUseCases, sdWirelessArch}.


%In parallel, the increasing attention to cloud computing due to its on-demand availability has triggered container focused development. In recent years a shift has been seen in computing from physical hardware to VMs, to VMs in the cloud \cite{vms} and finally to containers \cite{containers, vm_vs_container}. 
%Consequently, this has brought up the need to orchestrate and manage the containers in a way that can meet up the elasticity in scaling (horizontally and vertically), making Kubernetes almost the de-facto standard for automating these deployments.

At the same time, the \emph{compute} environment is following its own evolution. Compute granularity is increasing, from physical hardware to VMs, then to containers \cite{containers, vm_vs_container} and more recently towards Lambda functions \cite{serverlessEconomics, lambdaBenchmarking}. This  makes it possible to  consume resources more efficiently, as well as unprecedented scalabilty. In addition, it requires orchestration mechanisms to ease management and more importantly, to automatically scale up or down computing capacity depending on the load. This is often referred as autoscaling.



In this context, orchestration software to manage large pools of compute resources, such as OpenStack for virtual machines \cite{openStackArchitecture}, or Kubernetes for containers \cite{kubernetesConcepts} has become commonplace. Moreover, they have been naturally extended into the networking domain, especially in the case of service meshes, like Envoy proxies controlled by the Istio controller \cite{serviceMeshSoA}. However, all these extensions are limited to datacenter networks, and despite their extensibility and programmability they cannot reach beyond the datacenter network, notably into the networks (e.g., Wide-Area Networks WAN) interconnecting the datacenter with the end-users.

%However, the \emph{compute} and the \emph{networking} domains do not talk. 


This lack of communication between the cloud and the WAN hinders some of the advantages of the cloud.  A key limitation resulting from this lack of communication is in the context of cloud autoscaling events. Autoscaling is a cloud feature to dynamically adapt the amount of compute resources to the current load, as a way to improve efficiency and optimise cost. Usually, cloud autoscaling works in two axes. The first, vertical autoscaling (also known as scale up or down) refers to adding more resources to an existing cloud instance, such as CPU, memory or I/O resources. The second, horizontal autoscaling (scale out or in) involves adding new cloud instances to divide a workload among them.


In current data-centers and WANs, autoscaling events detected by the cloud orchestrator only propagate within the compute domain (i.,e, datacenter). Although an application can scale up to support higher loads, the connection towards the users remains unchanged, which might cause congestion or reduce QoE. Conversely, when applications scale down, network resources become idle and underutilised. 

%With this, autoscaling events detected by the cloud orchestrator only propagate within the compute domain (i.,e, datacenter), but not to the networking domain that connects the application with the end-users. This fundamentally limits the autoscaling properties of the cloud, since an application can scale up to support higher loads, but the connection towards the uses remains unchanged, which might cause congestion. Similarly, inefficient use the network resources occurs when the application scales down. 


%TODO: say clearly that usually the scaling is reactive, the most notable example are techniques in elastic optical networks. Say here we want to be proactive. This makes it possible to adapt to changing demands. 
Taking this into account, in this paper we argue that there is a need to develop the necessary abstractions and protocols to interconnect the \emph{compute} and the \emph{networking} domains, with a strong focus on the network autoscaling properties. This will enable matching the requirements of applications and services with the resources offered by the network, increasing the resource efficiency. 


In this paper we explore how to propagate cloud autoscaling events to the network that connects the datacenter with the end-users. For this, first we define vertical and horizontal network autoscaling and present a general architecture to support such new features. Then, we experimentally prototype and analyse two real-world use-cases of both network autoscaling scenarios. And finally, we take advantage of both experiments to derive open research challenges in this field.

